A Tight Analysis of the Parallel Undecided-State Dynamics with Two Colors

The \emph{Undecided-State Dynamics} is a well-known protocol for distributed consensus. We analyze it in the parallel \pull\ communication model on the complete graph for the \emph{binary} case (every node can either support one of \emph{two} possible colors, or be in the undecided state). An interesting open question is whether this dynamics \emph{always} (i.e., starting from an arbitrary initial configuration) reaches consensus \emph{quickly} (i.e., within a polylogarithmic number of rounds) in a complete graph with $n$ nodes. Previous work in this setting only considers initial color configurations with no undecided nodes and a large \emph{bias} (i.e., $\Theta(n)$) towards the majority color. In this paper we present an \textit{unconditional} analysis of the Undecided-State Dynamics that answers to the above question in the affirmative. We prove that, starting from \textit{any} initial configuration, the process reaches a monochromatic configuration within $O(\log n)$ rounds, with high probability. This bound turns out to be tight. Our analysis also shows that, if the initial configuration has bias $\Omega(\sqrt{n\log n})$, then the dynamics converges toward the initial majority color, with high probability.

==> trunk/apx-omittedproofs.tex <==
\section{Omitted proofs} \label{app:omittedproof}

\subsection{Proof of Claim~\ref{claim:s_increase}}
Recall that $S = A - B$. In order to show that $S>s(1 + \frac{1}{36})$ w.h.p., we provide two independent bounds to the values of $A$ and $B$, respectively. We use the additive form of the Chernoff bound ((\ref{eq:cbafleq}) and (\ref{eq:cbafgeq}) in Appendix \ref{apx:cbaf}) with $\lambda = \frac{\gamma\sqrt{n \log n}}{72}$. Hence, we have
%
\begin{align*}
\Prob{}{A \leq  \Expec{}{A \vert X_t = \x} - \lambda} &\leq e^{-2\lambda^2/n}\\ 
&= e^{-2\gamma^2 \log n/72^2}\\
&= \frac{1}{n^{\Theta(1)}},
\end{align*} 
%
\noindent and
%
\begin{align*}
\Prob{}{B \geq  \Expec{}{B \vert X_t = \x} + \lambda} &\leq e^{-2\lambda^2/n}\\ &= e^{-2\gamma^2 \log n/72^2}\\ &= \frac{1}{n^{\Theta(1)}}.
\end{align*} 
%
\noindent Then w.h.p.
%
\begin{align*}
S &>  \Expec{}{A \vert X_t = \x} - \lambda - [B \vert X_t = x] - \lambda\\
&= \Expec{}{A - B \vert X_t = \x} - 2 \lambda\\
&= \Expec{}{S \vert X_t = \x} - 2 \lambda\\
&= s(1 + \frac{q}{n}) - \frac{\gamma\sqrt{n \log n}}{36}\\
&\geq s(1 + \frac{q}{n}) - s/36\\
&\geq s(1 + \frac{1}{18} - \frac{1}{36})\\
&=s(1 + \frac{1}{36}).
\end{align*} 
%
We now show that $S<2s$ w.h.p. using similar arguments as above. Once again, we use the additive form of the Chernoff bound with $\lambda = \frac{\gamma\sqrt{n \log n}}{4}$. We have
%
\begin{align*}
\Prob{}{A \geq  \Expec{}{A \vert X_t = \x} + \lambda}& \leq e^{-2\lambda^2/n}\\ &= e^{-2\gamma^2 \log n/16}\\ &= \frac{1}{n^{\Theta(1)}},
\end{align*} 
\noindent and
%
\begin{align*}
\Prob{}{B \leq  \Expec{}{B \vert X_t = \x} - \lambda} &\leq e^{-2\lambda^2/n}\\ &= e^{-2\gamma^2 \log n/16}\\ &= \frac{1}{n^{\Theta(1)}}.
\end{align*} 
%
\noindent As a consequence, we have that w.h.p.
\begin{align*}
S &<  \Expec{}{A \vert X_t = \x} + \lambda - [B \vert X_t = x] + \lambda\\
&= \Expec{}{A - B \vert X_t = \x} + 2 \lambda\\
&= \Expec{}{S \vert X_t = \x} + 2 \lambda\\
&= s(1 + \frac{q}{n}) + \frac{\gamma}{2}\sqrt{n \log n}\\
&< s(1 + \frac{1}{2}) + \frac{1}{2}s\\
&=2s.
\end{align*}
\qed

\subsection{Proof of Claim~\ref{claim:b_decrease}}

W.l.o.g. we assume that $a>b$. From (\ref{eq:expdecrb}), since $s\geq \frac{2}{3}n$, we have that
%
\begin{align*} \Expec{}{B \, \vert \, X_t = \x} &= b \left( 1-\frac{2s+3b-n}{n} \right)\\
&\leq b \left( 1-\frac{2s-n}{n} \right)\\
&\leq b \left( 1-\frac{\frac{4}{3}n-n}{n} \right)\\
&= b \left( 1- \frac{1}{3}\right).
\end{align*}
%
\noindent
Then we apply the multiplicative form of the Chernoff Bound ((\ref{eq:cbmfgeq}) in Appendix \ref{apx:cbmf}) with $\delta = \frac{1}{3}$, and we obtain
%
\begin{align*}
\Prob{}{B \geq (1+\delta)\left( 1- \frac{1}{3}\right)b} &\leq e^{-b(1-\frac{1}{3})\delta^2/3}\\  
&\leq e^{-\log n(1-\frac{1}{3})\delta^2/3}\\ &= \frac{1}{n^{\Theta(1)}}.
\end{align*}
%
\noindent
As a consequence, we have that w.h.p.
%
\begin{align*}
B &\leq b(1+\delta)\left(1-\frac{1}{3}\right)\\ &= b\left(1+\frac{1}{3}\right)\left(1-\frac{1}{3}\right)\\
&= b \left(1-\frac{1}{9}\right).
\end{align*} \qed
%
\subsection{Proof of Claim~\ref{claim:s_preserved}}

W.l.o.g. we assume that $a>b$. We recall that $S = A - B$, thus we provide two independent bounds to the values of $A$ and $B$ respectively. We use the additive form of the Chernoff bound (see (\ref{eq:cbafleq}) and (\ref{eq:cbafgeq}) in Appendix \ref{apx:cbaf}) with $\lambda = \epsilon\frac{\sqrt{n \log n}}{2}$. We have
%
\begin{align*}\Prob{}{A \leq  \Expec{}{A \vert X_t = x} - \lambda}& \leq e^{-2\lambda^2/n}\\ &= e^{-\epsilon^2\log n/2}\\ &= \frac{1}{n^{\Theta(1)}},
\end{align*}
%
\noindent and
%
\begin{align*}\Prob{}{B \geq  \Expec{}{B \vert X_t = x} + \lambda}& \leq e^{-2\lambda^2/n}\\ &= e^{-\epsilon^2\log n/2}\\ &= \frac{1}{n^{\Theta(1)}}.
\end{align*}
%
\noindent Then it holds that, w.h.p.
%
\begin{align*}
S &\geq  \Expec{}{A \vert X_t = x} - \lambda - \Expec{}{B \vert X_t = x} - \lambda\\
&= \Expec{}{A - B \vert X_t = x} - 2 \lambda\\
&= \Expec{}{S \vert X_t = x} - 2 \lambda\\
&= s(1 + \frac{q}{n}) - \epsilon\sqrt{n \log n}\\
&\geq s + \frac{2\sqrt{n \log n}}{3} - \epsilon\sqrt{n \log n}\\
&>s
\end{align*} \qed

\subsection{Proof of Claim~\ref{claim:q_preserved}}

W.l.o.g. we assume that $a>b$. The number of \colB-colored nodes is at least $2\sqrt{n \log n}$ and each node has probability at least $2/3$ to pick an \colA-colored node. Thus $\Expec{}{Q} > \frac{4}{3}\sqrt{n \log n}$ and we get the claim by a simple application of the additive form of the Chernoff bound. \qed

%%%%%%%%%%%
\iffalse
\subsection{Proof of Claim~\ref{claim:q_does_not_increase}}

Let us first observe  that $s \geq \frac{2}{3}n$ implies that $q \leq \frac{1}{3}n$, which in turn implies $2q^2 + (n-q)^2 < n^2$. Hence, using (\ref{eq:explbq}), we get
\begin{align}
\Expec{}{Q \, \vert \, X_t = \x} &= \frac{2q^2 + (n-q)^2 - s^2}{2n}\nonumber\\
&\leqslant \frac{n}{2} - \frac{s^2}{2n}\\
&\leqslant \frac{n}{2} - \frac{2}{9}n\nonumber\\
&= \frac{5}{18}n. \nonumber
\end{align}
\noindent We can now  apply the additive form of the Chernoff Bound ((\ref{eq:cbafleq}) and (\ref{eq:cbafgeq}) in Appendix \ref{apx:cbaf}) with $\lambda = \frac{1}{18}$. We finally get 

\[\Prob{}{Q \geq \frac{1}{6}n} = \Prob{}{Q \geq \frac{5}{18}n + \frac{1}{18}n} \leq  \Prob{}{Q \geq \Expec{}{Q} + \frac{1}{18}n} \leq e^{-2n^2/18^2n} = e^{-\Theta(n)}.\] \qed
\fi
%%%%%%%%%%%%


\subsection{Proof of Claim~\ref{claim:q_decrease}}

From (\ref{exp:q}), we have:
%
\begin{align*}
\Expec{}{Q\vert X_t = \x} &= \frac{q^2 + 2ab}{n} \leq \frac{q^2 + 4 n \sqrt{n \log n}}{n}\\ &= q( \frac{q}{n} + \frac{4 \sqrt{n \log n}}{q})\\ 
&\leq q(\frac{1}{3} + \frac{1}{3})\\ &= q(1 - \frac{1}{3}).
\end{align*}
%
\noindent Thus we apply the multiplicative form of the Chernoff Bound (\ref{eq:cbmfgeq} in Appendix \ref{apx:cbmf}) with $\delta = \frac{1}{3}$
%
\begin{align*}
\Prob{}{Q \geq (1+\delta)\left( 1- \frac{1}{3}\right)q} &\leq e^{-q(1-\frac{1}{3})\delta^2/3}\\
&\leq e^{-\log n(1-\frac{1}{3})\delta^2/3}\\
&= \frac{1}{n^{\Theta(1)}},
\end{align*}
%
\noindent and thus we get that, w.h.p.,

\[Q \leq \left(1 + \frac{1}{3}\right)\left( 1- \frac{1}{3}\right)q = q\left( 1- \frac{1}{9}\right). \] 
 \qed


\subsection{Proof of Claim~\ref{claim:a_wins}}

We first show that in one round the number of nodes that support   color \colB\ becomes logarithmic 
and the number of undecided nodes does not increase.
%
\begin{align*}
\Expec{}{B \, \vert \, X_t = \x}& = b\left(\frac{b + 2 q}{n} \right)\\ &\leq 2\sqrt{n \log n}\left(\frac{2\sqrt{n \log n} + 2 \gamma \sqrt{n \log n}}{n}\right)\\ &= 4(\gamma +1) \log n.
\end{align*}
%
Using the multiplicative form of the Chernoff bound we  get that $B < 8(\gamma +1) \log n$, w.h.p. We now show that the number of the undecided nodes is still $\bigO(\sqrt{n \log n})$. Indeed
%
\begin{align*}
\Expec{}{Q \, \vert \, X_t = \x}& = \frac{q^2}{n} + \frac{2ab}{n}\\ &\leq \gamma^2 \log n + 4 \sqrt{n \log n}.
\end{align*}
%
Then using the additive form of the Chernoff bound we get that $Q \leq 5 \sqrt{n \log n} $ ,w.h.p. In the next round, w.h.p., no undecided node picks a node colored of \colB\ or vice versa, so we can conclude that there are no nodes that still support \colB\   (and it easy to show that there is at least one supporter of \colA\, w.h.p.). From now on, the stochastic process is equivalent to the  classic spreading process via \pull\ operations, and thus, within $\bigO(\log n)$ rounds, all the nodes will support \colA\ w.h.p. \qed

\subsection{Proof of Claim~\ref{claim:s_does_not_decrease}}

Since $S = A - B$,   we need to  provide two   bounds to the values of $A$ and $B$, respectively. We use the additive form of the Chernoff bound ((\ref{eq:cbafleq}) and (\ref{eq:cbafgeq}) in Appendix \ref{apx:cbaf}) with $\lambda = \epsilon\frac{\sqrt{n \log n}}{2})$. We have

\[\Prob{}{A \leq  \Expec{}{A \vert X_t = x} - \lambda} \leq e^{-2\lambda^2/n} = e^{-\epsilon^2\log n/2} = \frac{1}{n^{\Theta(1)}},\]

\noindent and

\[\Prob{}{B \geq  \Expec{}{B \vert X_t = x} + \lambda} \leq e^{-2\lambda^2/n} = e^{-\epsilon^2\log n/2} = \frac{1}{n^{\Theta(1)}}.\]

\noindent Then it holds that, w.h.p.,
%
\begin{align*}
S &\geq  \Expec{}{A \vert X_t = x} - \lambda - \Expec{}{B \vert X_t = x} - \lambda\\
&= \Expec{}{A - B \vert X_t = x} - 2 \lambda\\
&= \Expec{}{S \vert X_t = x} - 2 \lambda\\
&= s(1 + \frac{q}{n}) - \epsilon\sqrt{n \log n}\\
&\geq s - \epsilon\sqrt{n \log n}\\
&\geq\gamma\sqrt{n \log n} - \epsilon\sqrt{n \log n}\\
&=(\gamma-\epsilon)\sqrt{n \log n}.
\end{align*}\qed

%%%%PUT IN THE BODY

\iffalse
\subsection{Tightness of Theorem \ref{thm:mainmajority}}\label{proof:tightness}

\begin{claim}\label{claim:apxminbias} An initial configuration exists with $\abs{s} = \Theta(\sqrt{n})$ such that the process converges to the minority color with constant probability.
\end{claim}

\begin{proof}
Let us consider the configuration $\x$ such that $q(\x) = n/3, a(\x) = n/3 + \sqrt{n}$ and $b(\x) = n/3 - \sqrt{n}$. We prove that in one round there is constant probability that the bias becomes zero or negative. After that, by a simple symmetry argument, we get the claim.

We define $A^q,B^q,Q^q$ the random variables counting the nodes that were undecided in the configuration $\x$ and that, in the next round, 
get    colored with  \colA, \colB\ ,or undecided, respectively. Similarly $A^a$ ($B^b$) counts the nodes that    supported
   color \colA\ (\colB) in the configuration $\x$ and that, in the next round,    still support the same color.

Since it is impossible that a node supporting a color  gets the other color in the next round, it holds that $A = A^q + A^a$ and $B = B^q + B^b$. Moreover, observe  that, among these random variables, only $A^q$ and $B^q$ are mutually dependent. Thus, for any positive constant $\delta$, it holds  
\begin{align*}
&\Prob{}{S \leq 0} = \Prob{}{B \geq A}\\
&= \Prob{}{B^q + B^b \geq A^q + A^a}\\
&\geq \Prob{}{B^q \geq A^q \, , \, B^b \geq n/3 + \delta\sqrt{n}  \, , \,  A^a \leq n/3 + \delta\sqrt{n}}\\
&= \Prob{}{B^q \geq A^q} \cdot \Prob{}{B^b \geq n/3 + \delta\sqrt{n}}\\ &\,\,\,\,\cdot \Prob{}{A^a \leq n/3 + \delta\sqrt{n}}.
\end{align*}
By  applying   the Reverse Chernoff bound (see~(\ref{eq:rcbgeq})), we get that $\Prob{}{B^b \geq n/3 + \delta\sqrt{n}}$ is at least constant, 	whereas the fact that $\Prob{}{A^a \leq n/3 + \delta\sqrt{n}}$ is at least constant is an immediate consequence of the additive form of the Chernoff Bound (see~\eqref{eq:cbafgeq}). 

Thus we need to show that   $\Prob{}{B^q \geq A^q}$ is at least constant, as well.
 Note that the distribution $B^q$ conditioned to the event $Q^q = k$ is a binomial distribution with parameters $(\frac{n}{3}-k,\frac{b(\x)}{a(\x)+b(\x)})$ and with expectation $\Expec{}{B^q \, \vert \, Q^q = k, X_t = \x} = (\frac{n}{3}-k)/2 - (\frac{n}{3}-k)/(6\sqrt{n})$. Thus we get
%
\allowdisplaybreaks 
\begin{align}
&\Prob{}{B^q \geq A^q} = \sum_{k=1}^{n/3} \Prob{}{B^q \geq A^q \, \vert \, Q^q = k}\Prob{}{Q^q = k}\nonumber\\
&> \sum_{k=n/4}^{n/2} \Prob{}{B^q \geq A^q \, \vert \, Q^q = k}\Prob{}{Q^q = k}\nonumber\\
&= \sum_{k=n/4}^{n/2} \Prob{}{B^q \geq (\frac{n}{3} - k)/2) \, \vert \, Q^q = k}\Prob{}{Q^q = k}\nonumber\\
&= \sum_{k=n/4}^{n/2} \Prob{}{B^q \geq \substack{\Expec{}{B^b\, \vert \, Q^q = k}\\ + (\frac{n}{3}-k)/(6\sqrt{n})} \, \vert \, Q^q = k}\Prob{}{Q^q = k}\nonumber\\
&= \sum_{k=n/4}^{n/2} \Prob{}{B^q \geq \substack{\Expec{}{B^b\, \vert \, Q^q = k} \\ \cdot(1 + \frac{1}{3\sqrt{n}-1})} \, \vert \, Q^q = k}\Prob{}{Q^q = k}\nonumber\\
&\geq \sum_{k=n/4}^{n/2} \exp\left(\frac{-9}{(3\sqrt{n}-1)^2} \cdot \Expec{}{B^b\, \vert \, Q^q = k}\right)\Prob{}{Q^q = k}\label{appliedreverse}\\
&\geq \sum_{k=n/4}^{n/2} \exp\left(\frac{-9n}{(3\sqrt{n}-1)^2} \right)\Prob{}{Q^q = k}\nonumber\\
&= \exp\left(\frac{-9n}{(3\sqrt{n}-1)^2} \right) \sum_{k=n/4}^{n/2} \Prob{}{Q^q = k}\nonumber\\
&= \Theta(1) \sum_{k=n/4}^{n/2} \Prob{}{Q^q = k}\nonumber\\
&=\Theta(1) (1 - e^{-\Theta(n)}), \label{concentrateq}
\end{align}
where in (\ref{appliedreverse}) we used the reverse Chernoff bound (see~(\ref{eq:rcbgeq})) and in (\ref{concentrateq}) we used that $\Expec{}{Q^q} \approx \frac{n}{3}$ and the additive form of the Chernoff bound. 
\end{proof}
\fi


==> trunk/apx-symmetry.tex <==
\section{Proof of the Symmetry Breaking Lemma (Lemma~\ref{lemma:symmetrygeneric})} \label{apx:symmbreak}

For the sake of brevity we define $Y_t = f(X_t)$. We define a stochastic process $\{Z_t\}_t$ such that $Z_t = Y_t^2 - t\delta^2$. We first show this new stochastic process is a supermartingale:
\begin{align}
\Expec{}{Z_{t+1}\vert X_t= \x}\nonumber  
&= \Expec{}{Y_{t+1}^2\vert X_t= \x} - (t+1) \delta^2 \nonumber\\ 
&= \Expec{}{Y_{t+1}\vert X_t= \x}^2 + \Var{}{Y_{t+1} \vert X_t= \x} - (t+1) \delta^2 \nonumber\\ 
&\geq \Expec{}{Y_{t+1}\vert X_t= \x}^2 + \delta^2 - (t+1) \delta^2 \nonumber\\ &\geq \Expec{}{Y_{t+1}\vert X_t= \x}^2 - t \delta^2 \nonumber\\ 
&\geq f(X_t)^2 - t \delta^2  \label{eq:super}  \\
&= Y_t^2 - t \delta^2\nonumber\\
&= Z_t\nonumber
\end{align}

Where in (\ref{eq:super}) we used the Assumption \ref{ass:outdrift}. It is clear that $\tau$ is a stopping time, and we show it meets the conditions of the Optional Stopping Theorem \cite[Corollary 17.7]{lpw08}. Indeed: 

$$\Expec{}{Y_{t+1}^2 \vert X_t= \x} = \Var{}{Y_{t+1} \vert X_t= \x} + \Expec{}{Y_{t+1} \vert X_t= \x}^2 \geq \delta^2 + f(\x)^2$$

The expectation $\Expec{}{Y_{t+1}^2 \vert X_t= \x}$ can we rewritten in the following way:
\begin{align*}
\Expec{}{Y_{t+1}^2 \vert X_t= \x} &= \Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \leq i }\Prob{}{Y_{t+1} \leq i \vert X_t= \x}\\ &+\Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \geq i}\Prob{}{Y_{t+1} \geq i + 1 \vert X_t= \x } \\
&\geq \delta^2 + f(\x)^2
\end{align*}

Now we focus on the probability of reaching a configuration $\x'$ such that $\vert f(\x') \vert \geq i + 1$:

\begin{align*}
\Prob{}{Y_{t+1} \geq i + 1 \vert X_t= \x } &\geq  \frac{\delta^2 + f(\x)^2 - \Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \leq i }\Prob{}{Y_{t+1} \leq i}}{\Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \geq i}} \\ &\geq \frac{\delta^2 + f(\x)^2 - \Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \leq i }}{\Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \geq i}} \\ &\geq \frac{\delta^2 + f(\x)^2 - i^2}{\Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \geq i}}
\end{align*}

Then, for any $x$ such that $f(\x) = i \geq 0$:

$$\Prob{}{Y_{t+1} \geq i + 1 \vert X_t= \x \wedge f(\x) = i} \geq \frac{\delta^2 + i^2 - i^2}{\Expec{}{Y_{t+1}^2 \vert X_t= \x \wedge Y_{t+1} \geq i}} \geq \frac{\delta^2}{n^2}= \epsilon$$

Where $\epsilon$ is a positive constant (it does not depend on $t$). This means that the r.v.\ representing the unbalance have always a constant positive probability of increase of one step, round by round. Thus starting from any state $x \in A$ such that $\vert f(\x) \vert \leq m-1$ it easy to see after $m$ rounds the probability $\Prob{x}{\tau \leq m} \geq \epsilon^m$. Hence:

$$\Expec{x}{\tau} = \sum_{i=0}^{\infty} \Prob{x}{\tau \geq i} \leq \sum_{i=0}^{\infty} m \Prob{x}{\tau \geq i m} \leq \sum_{i=0}^{\infty} m (1-\epsilon^m)^i < \infty$$


%%%%%%%%%%%%%%%%%%%%%
 
As for the second condition of the Optional Stopping Theorem, it is clear that for any $\x \in \mathcal{C}$ we have $\Expec{}{\vert Y_{t+1} - Y_t \vert \, \vert \,  X_t = \x} \leq 2n$ (the stochastic process $\{Y_t\}_{t \in \mathbb{N}}$ in defined in $[-n,n]$), thus we can apply the bound on the expectation of the supermartingale $\{Z_t\}_t$ to the stopping time $\tau$ and we get
\begin{equation*}
\Expec{}{Z_\tau} \geq \Expec{}{Y_\tau^2} - \Expec{}{\tau}\delta^2 \geq \Expec{}{Z_0} \geq 0
\end{equation*}
\begin{equation*}
\Expec{}{\tau} \leq \Expec{}{Y_\tau^2}/\delta^2
\end{equation*}
\qed


==> trunk/expander.tex <==
\section{Expanders}

The proof of previous section heavy relies on the assumption of a underlying complete graph. In this section we generalize the previous results on the class of $d$-regular graphs. In a generic graph $G(V,E)$ the configuration of the process can not be expressed only in terms of cardinalities of the nodes supporting the different colors, but we also need to know where these nodes are. In any round $t$ the configuration $X_t \in \mathcal{C}$ of the \threestateprocess\ on a generic graph $G(V,E)$ is defined by the set of nodes the support the first color (e.g. the \colA\ one) $A_t \subseteq V$, the set of nodes the support the second color (e.g. the \colB\ one) $B_t \subseteq V$, the remaining set of undecided nodes $Q_t \subseteq V$ (i.e. $X_t = (A_t,B_t,Q_t)$). We again define the bias as $s_t = \vert A_t \vert - \vert B_t \vert$. In order to use a shorter notation we use the minuscule letter to refer the cardinality of the set (e.g $\card{A_t} = a_t$). When there are no ambiguities we make use of the following short notations: $A' = A_{t+1}$, $A = A_t$ and $a = a_t$.\\

Let $G(n,d,\lambda)$ be a $d$-regular graph for which $\lambda = \lambda(G) = \max(\abs{ \lambda_2}, \abs{ \lambda_n })$ where $\lambda_i$ is the $i$-th eigenvalue of the adjacency matrix of $G$. Let $E(S,T)$ be the number of edges that have a vertex in $S$ and the other in $T$. For this kind of graphs the following Expander Mixing Lemma bounds the number of edges between any two sets of vertices:

\begin{lemma}[The Expander Mixing Lemma]
Let $G$ be a $G(n,d,\lambda)$ graph. Then for all $S, T \subseteq V$:

$$\abs{\,\card{E(S,T)}- \frac{d\card{S}\card{T}\,}{n}} \leq \lambda\sqrt{\card{S}\,\card{T}}$$
\end{lemma}

We can represent any configuration $X_t \in \mathcal{C}$ as in Figure \ref{fig:config}. The label of the edge counts the number of the edges intra and inter the components defined by $A,B$ and $Q$. We define $\delta_{S,T} := E(S,T)- \frac{d}{n}\card{S}\card{T}$. When we write $\delta_{S}$ we mean $\delta_{S,S}$ Thanks to the above Lemma we can say that, for any $X,Y \in [A,B,Q]$:

\[\delta_{X,Y} \in [ -\lambda\sqrt{\vert X \vert \cdot \vert Y \vert},\lambda\sqrt{\vert X \vert \cdot \vert Y \vert} ] \]
Moreover, because the graph is regular
\[\delta_{A,B} + \delta_{A,Q} + \delta_A = 0\]
\[\delta_{A,B} + \delta_{B,Q} + \delta_B = 0\]
\[\delta_{A,Q} + \delta_{B,Q} + \delta_Q = 0\]


\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.5]{./imgs/dregular.png}
\end{center}
\caption{A representation of a generic configuration $X \in \mathcal{C}$ }
\label{fig:config}
\end{figure}

This representation does not fully define the configuration $X_t$ (we do not know how exactly the nodes are connected) but it is sufficient to define the expectation of the cardinalities of the different sets. We call $\Expec{}{S\rightarrowtail T}$ the expected number of nodes in $S$ that see a node in $T$ in a given round, with $S,T \subseteq V$. $N(v,S)$ is the number of neighbours of $v$ that are in $S$. We can now write the expectation of the cardinalities of the different sets.

\begin{align}
\Expec{}{ \card{A'} \vert X_t = (A,B,Q)}  &= \Expec{}{A\rightarrowtail (A\cup Q) \vert X_t= (A,B,Q)} + \Expec{}{Q\rightarrowtail A \vert X_t = (A,B,Q)}\nonumber \\
&= \sum_{v \in A} \frac{N(v,A \cup Q)}{d} + \sum_{u \in Q} \frac{N(u,A)}{d}\nonumber \\
&=  \frac{E(A,A \cup Q)}{d} +  \frac{E(Q,A)}{d}\nonumber\\
&= \frac{\frac{d}{n}a^2 + \delta_A + \frac{d}{n}aq + \delta_{A,Q}}{d} + \frac{\frac{d}{n}aq + \delta_{A,Q}}{d}\nonumber \\
&= \frac{a^2}{n} + 2\frac{aq}{n} + \frac{\delta_A + 2\delta_{A,Q}}{d}\nonumber \\
&= a \left( \frac{a + 2q}{n} \right) + \frac{\delta_{A,Q} - \delta_{A,B}}{d}\label{expander1}
\end{align}

where in (\ref{expander1}) we used that $\delta_{A,Q}= - \delta_A - \delta_{A,B}$. The same result can be obtained for $\card{B}$. Moreover:

\begin{align}
\Expec{}{ \card{S'} \vert X_t = (A,B,Q)} &= \Expec{}{ \card{A'} \vert X_t = (A,B,Q)} - \Expec{}{ \card{B'} \vert X_t = (A,B,Q)} \\
&= a \left( \frac{a + 2q}{n} \right) + \frac{\delta_{A,Q} - \delta_{A,B}}{d} - b \left( \frac{b + 2q}{n} \right) + \frac{\delta_{B,Q} - \delta_{A,B}}{d}\\
&= s \left( 1 + \frac{q}{n} \right) + \frac{\delta_{A,Q} - \delta_{B,Q}}{d}
\end{align}

Also $\card{Q}$ admits a similar expectation:
\begin{align}
\Expec{}{\card{Q'} \vert X_t = (A,B,Q)} &= \Expec{}{q \rightarrowtail q} + \Expec{}{a \rightarrowtail b} + \Expec{}{b \rightarrowtail a} \\
&= \frac{E(Q,Q) + E(A,B) + E(B,A)}{d} \\
&= \frac{q^2 + 2ab}{n} + \frac{\delta_{Q} + 2 \delta_{A,B}}{d}
\end{align}

All the results of previous section rely the following claims: Claim \ref{claim:q_lower_bound}, Claim \ref{claim:s_increase}, Claim \ref{claim:b_decrease}, Claim \ref{claim:q_decrease}, Claim \ref{claim:s_does_not_decrease}. If $s = \omega(\frac{\lambda}{d}n)$:

\begin{align}
\Expec{}{\card{S'} \vert X_t = (A,B,Q))} &= s \left( 1 + \frac{q}{n} \right) + \frac{\delta_{A,Q} - \delta_{B,Q}}{d} \\
&= s \left( 1 + \frac{q}{n} \right) + O(\frac{\lambda(\sqrt{aq}+\sqrt{bq})}{d})\\
& = s \left( 1 + \frac{q}{n} \right) + O(\frac{\lambda}{d}n)\\
&= s \left( 1 + \frac{q}{n} \pm \epsilon \right)
\end{align}

for any $\epsilon > 0$. If $a = \omega((\frac{\lambda}{d})^2n)$:

\begin{align}
\Expec{}{\card{A'} \vert X_t = (A,B,Q))}  &= a \left( \frac{a + 2q}{n} \right) + \frac{\delta_{A,Q} - \delta_{A,B}}{d} \\
&= a \left( \frac{a + 2q}{n} \right) + O( \frac{\lambda (\sqrt{aq} + \sqrt{ab})}{d}) \\
&= a \left( \frac{a + 2q}{n} \right) + O( \frac{\lambda\sqrt{a}\sqrt{n})}{d}) \\
&= a \left( \frac{a + 2q}{n}  + O( \frac{\lambda\sqrt{n})}{d\sqrt{a}}) \right)\\
&= a \left( \frac{a + 2q}{n}  \pm \epsilon \right)
\end{align}

for any $\epsilon > 0$.  if $q = \omega(\frac{\lambda}{d}n)$.

\begin{align}
\Expec{}{\card{Q'} \vert X_t = (A,B,Q))}  &= \frac{q^2 + 2ab}{n} + \frac{\delta_{Q} + 2 \delta_{A,B}}{d} \\
&= q \left( \frac{q}{n}+\frac{2ab}{qn} \right) + O \left( \frac{\lambda (q +\sqrt{a b})}{d} \right) \\
&= q \left( \frac{q}{n}+\frac{2ab}{qn} \right) + O \left( \frac{\lambda n}{d} \right) \\
&= q \left( \frac{q}{n}+\frac{2ab}{qn} \pm \epsilon \right)
\end{align}

for any $\epsilon > 0$. 
